Verifying C11 Programs Operationally

This paper develops an operational semantics for a release-acquire fragment of the C11 memory model with relaxed accesses. We show that the semantics is both sound and complete with respect to the axiomatic model. The semantics relies on a per-thread notion of observability, which allows one to reason about a weak memory C11 program in program order. On top of this, we develop a proof calculus for invariant-based reasoning, which we use to verify the release-acquire version of Peterson's mutual exclusion algorithm.

==> peterson.tex <==

\newcommand{\defn}{\mathrel{\widehat{=}}}

\newcommand{\flag}{\mathit{flag}}
\newcommand{\turn}{\mathit{turn}}

% \section{Peterson's algorithm}

\begin{example}[Peterson's algorithm]
The running example for this paper will be the classic Peterson's
mutual exclusion algorithm for two processes (see
\refalg{alg:petersons-ra}) implemented using release-acquire annotations.
As with the original algorithm, variable $\flag_i$ is used to indicate
whether process $i$ intends to enter its critical section and a shared
variable $\turn$ is used to ``give way'' when both processes intend to
enter their critical sections at the same time.

We describe the algorithm for process $0$; the other process is
symmetric.  The flag variable is set to $\True$ (line \ref{set-flag})
using relaxed atomics (which does not induce any synchronisation), but
is set to $\False$ (line \ref{unset-flag}) using a release
annotation. The intention of the latter is to synchronise this write
(of $\False$ to $\flag$) with the read of $\flag_0$ at
line \label{busy-wait} in process $1$. The value of $\turn$ is set
using a $\kwswap$
command. % This means that all executions of $\kwswap$ are totally
% ordered. 
Note however, that the read of $\turn$ within the guard of
the busy wait loop (line~\ref{busy-wait}) is relaxed. However, as we
shall see, the algorithm still satisfies the mutual exclusion
property.


\begin{algorithm}[!t]
  \caption{Peterson's algorithm with release-acquire
    synchronisation}\label{alg:petersons-ra}
\algrenewcommand\algorithmicindent{0.75em}
\begin{varwidth}[t]{0.49\columnwidth}
  \begin{algorithmic}[1] \small
    \Thread{0}
    % \While {true}
    \State $\flag_0$ := $\True$ ; \label{set-flag}
    \State $\turn$.\kwswap(\True)$^{\sf RA}$ ; \label{swap-turn} 
    \While {($\flag_1$ = \True)$^{\sf A}$ $\land$ $\turn$ = 1} \label{busy-wait}
    % \Statex \qquad \quad 
    \Skip
    \EndWhile 
    \State Critical section ; \label{critical-section}
    \State $\flag_0$ :=$^{\sf R}$ \False ; \label{unset-flag}
    % \EndWhile
    \EndThread
  \end{algorithmic}
\end{varwidth}
\hfill
\begin{varwidth}[t]{0.49\columnwidth}
  \begin{algorithmic}[1]
    \Thread{1}
    % \While {true}
    \State $\flag_1$ := \True ; 
    \State $\turn$.\kwswap(0)$^{\sf RA}$ ; 
    \While {($\flag_0$ = \True)$^{\sf A}$ $\land$ $\turn$ = 0}
    % \Statex \qquad \quad
    \Skip
    \EndWhile
    \State Critical section ;
    \State $\flag_1$ :=$^{\sf R}$ \False ;
    % \EndWhile
    \EndThread
  \end{algorithmic}
\end{varwidth}
\end{algorithm}

\end{example}



% A {\em configuration} $(P,\sigma)$ consists of a program $P$ and
% $\sigma \in \Sigma$. The command part of a configuration triggers
% operations on the memory model.  While the command language is however
% agnostic to values, the memory model will only allow certain values in
% read operations. This idea is captured by the following two rules
% combining commands and memory model.
% \[ \mathbf{Unrl}~\inference{C \ltsArrow{\tau}_t C'}{(C,\sigma) \ltsArrow{\tau}_t (C',\sigma)} \]  
% \[ \mathbf{Step}~\inference{C \ltsArrow{a}_t C' \quad \sigma \strans{\
%       e\ } \sigma' \quad act(e) = a \quad \tid(e) = t} {(C,\sigma)
%     \ltsArrow{a}_t (C',\sigma')} \] \hw{might we want the event e to
%   be visible in the combination?}

% \noindent Rule {\bf Unrl} describes a $\tau$-step of a thread and thus does not change the state of the memory model. 
% Rule {\bf Step} states that a thread can execute a specific operation $a$ in the current state $\sigma$ 
% only if the memory model in its transition relation permits it. 








% P0: flag[0] =_X true;   // (relaxed read)
%     turn.swap(1, rel_acq); // so it's a release/acquire swap, which reads and writes unconditionally
%     while (flag[1] ==_A true && turn ==_X 1)  // flag read is acquire, turn read is relaxed
%     {
%         // busy wait
%     }
%     // critical section
%     ...
%     // end of critical section
%     flag[0] =_R false;   // (releasing write)


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "hvc"
%%% End:



==> soundness-rules.tex <==
% !TeX root = ppopp.tex

\subsection{Soundness of Proof Rules in Figure \ref{fig:det-val-ind}}

We prove the soundness of all rules in Fig.~ \ref{fig:det-val-ind}. 
Thus, we consider the following setting (see caption of figure): 
In every rule, the variables $\sigma, m, e, \sigma'$
  satisfy $(\_,\sigma) \ltsArrow{m, e}_{C11} (\_,\sigma')$.  \hw{$tid(e) = t$?} 

\begin{description}
\item[NoMod] In state $\sigma$, we have $\OW_\sigma(t,x) = \{\sigma.\last(x)\}$ 
    (by definition of $x \detval{\sigma}_t v$). Since $e \notin \W_{|x}$, 
        $\OW_\sigma(t) = \OW_{\sigma'}(t)$ and 
       $\sigma.\last(x) = \sigma'.\last(x)$ and hence $\wrval(\sigma.\last(x)) = 
       \wrval(\sigma'.\last(x))$. 
       Furthermore, if $(\sigma.\last(x),e_t) \in \sigma.\lthb^?$ for some $e_t$ 
       with $\tid(e) = t$, then
       $(\sigma'.\last(x),e) \in \sigma'.\lthb)$ (as $(e_t,e) \in \sigma'.\ltsb$, thread order). 
\item[NoModOrder] If $e$ is neither modifying $x$ nor $y$, it is not changing $\last(x)$ and 
    $\last(y)$, nor their $\lthb$-order. 
\item[ModLast] If $(\_,\sigma) \ltsArrow{m, e}_{C11} (\_,\sigma')$, then 
    $m \in \OW_\sigma(t) \setminus \CW_\sigma(t)$. If $m = \sigma.\last(x)$, 
    then $e=\sigma'.\last(x)$. Furthermore, $e \in \observedWrites_{\sigma'}(t)$, 
    hence $m\notin \OW_{\sigma'}(t)$, but $e$ is and $\OW_{\sigma'}(t,x) = \{e\}$. 
    In addition, $(e,e) \in \lthb^?$ which completes all conditions necessary for 
   $x \detval{\sigma'}_t \wrval(e)$. 
\item[AcqRd] In this case, $e$ reads from $m$ and by this introduces an $\ltsw$ order due 
   to the release and acquire annotations. Because $e$ is a read, $m=\sigma'.\last(x)$ holds. 
   As $(m,e) \in \sigma'.\ltsw$, $(m,e) \in \sigma'.\lthb$. Moreover, $\rdval(e) = \wrval(m)$, 
   hence $\rdval(e) = \wrval(\sigma'.\last(x))$. 
\end{description} 


